StepFormer: Self-supervised Step Discovery and Localization in Instructional Videos

Instructional videos are an important resource to learn procedural tasks from human demonstrations. However, the instruction steps in such videos are typically short and sparse, with most of the video being irrelevant to the procedure. This motivates the need to temporally localize the instruction steps in such videos, i.e. the task called key-step localization. Traditional methods for key-step localization require video-level human annotations and thus do not scale to large datasets. In this work, we tackle the problem with no human supervision and introduce StepFormer, a self-supervised model that discovers and localizes instruction steps in a video. StepFormer is a transformer decoder that attends to the video with learnable queries, and produces a sequence of slots capturing the key-steps in the video. We train our system on a large dataset of instructional videos, using their automatically-generated subtitles as the only source of supervision. In particular, we supervise our system with a sequence of text narrations using an order-aware loss function that filters out irrelevant phrases. We show that our model outperforms all previous unsupervised and weakly-supervised approaches on step detection and localization by a large margin on three challenging benchmarks. Moreover, our model demonstrates an emergent property to solve zero-shot multi-step localization and outperforms all relevant baselines at this task.

==> bibref_long.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})



@string{iccv = "Proceedings of the International Conference on Computer Vision (ICCV)"}
@string{iccvw = "Proceedings of the International Conference on Computer Vision Workshops (ICCVW)"}
@string{eccv = "Proceedings of the European Conference on Computer Vision (ECCV)"}
@string{iclr = "International Conference on Learning Representations (ICLR)"}
@string{cvpr = "Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)"}
@string{bmvc = "British Machine Vision Conference (BMVC)"}
@string{nips = "Advances in Neural Information Processing Systems (NeurIPS)"}
@string{neurips = "Advances in Neural Information Processing Systems (NeurIPS)"}
@string{pami = "IEEE transactions on Pattern Analysis and Machine Intelligence (PAMI)"}
@string{ijcv = "International Journal of Computer Vision (IJCV)"}
@string{icml = "International Conference on Machine Learning (ICML)"}
@string{aaai = "AAAI Conference on Artificial Intelligence"}
@string{icra = "IEEE International Conference on Robotics and Automation (ICRA)"}
@string{icassp = "IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)"}
@string{eccvw = "Proceedings of the European Conference on Computer Vision Workshops (ECCVW)"}
1
